Learning and Adapting Agile Locomotion Skills by Transferring Experience

Legged robots have enormous potential in their range of capabilities, from navigating unstructured terrains to high-speed running. However, designing robust controllers for highly agile dynamic motions remains a substantial challenge for roboticists. Reinforcement learning (RL) offers a promising data-driven approach for automatically training such controllers. However, exploration in these high-dimensional, underactuated systems remains a significant hurdle for enabling legged robots to learn performant, naturalistic, and versatile agility skills. We propose a framework for training complex robotic skills by transferring experience from existing controllers to jumpstart learning new tasks. To leverage controllers we can acquire in practice, we design this framework to be flexible in terms of their source -- that is, the controllers may have been optimized for a different objective under different dynamics, or may require different knowledge of the surroundings -- and thus may be highly suboptimal for the target task. We show that our method enables learning complex agile jumping behaviors, navigating to goal locations while walking on hind legs, and adapting to new environments. We also demonstrate that the agile behaviors learned in this way are graceful and safe enough to deploy in the real world.

==> sections/finetune_algo.tex <==
\begin{algorithm}[t]
  	\caption{\footnotesize Fine-Tune}
  	\label{alg:finetune}
  	\begin{algorithmic}[1]{
\footnotesize
  	 \Require $\buff_\text{pre-train}$, $\policy_\theta$, and $Q_\theta$ from pre-training. Sampling ratio $\phi$. 
  	 \State Initialize: Replay buffer $\buff_\text{online}$.
    \item[]
        \State {{\textsc{// Fine-tune on all data using off-policy RL}}}
  	\Repeat
      	\State Collect data with $\policy_\theta(a \mid s)$.
      	\State Add experience to online buffer $\buff_\text{online} \leftarrow (s, a, s', r)$
            \State Update $Q_\theta$ and $\policy_\theta$, sampling $\phi$ from $\buff_\text{pre-train}$ and $(1-\phi)$ from $\buff_\text{online}$  
  	\Until{converged}
        }
  	\end{algorithmic}
\end{algorithm}

==> sections/pretrain_algo.tex <==
\begin{algorithm}[t]
  	\caption{\footnotesize Pre-Train}
  	\label{alg:pretrain}
  	\begin{algorithmic}[1]{
\footnotesize
          \Require $\text{MDP}\coloneqq(\statespace, p, \actionspace, r)$ of the desired task, \\and (optionally) narrow behavior policy $\policy_{\text{e}}$ with $\text{MDP}_\text{e}\coloneqq (\statespace_{\text{e}}, p, \actionspace, r_{\text{e}})$. 
  	 \State Initialize: Replay buffer $\buff$, Q-function $Q_\theta$ , and policy $\policy_\theta$.
    \item[]
  	\State {{\textsc{// (Optional) Initialize replay buffer using }$\policy_{\text{expert}}$}} 
  	\For{trajectory $i=0, 2, \dots, N_\text{seed trajectories}$}
            \State Roll out $\policy_{\text{e}}(a \mid s_\text{e})$ in $\text{MDP}_\text{e}$, recording actions $\{a_t\}_{t=1}^H$
            \State Collect $\traj=\{(s_t, a_t, s_{t+1}, r_t)\}_{t=1}^H$ in MDP by replaying $\{a_t\}_{t=1}^H$
            \State Add experience to buffer $\buff \leftarrow \traj$
      \EndFor

    \item[]
  	\State {{\textsc{// Pre-train using off-policy RL}}}
  	\Repeat
      	\State Collect data with $\policy_\theta(a \mid s)$.
      	\State Add experience to buffer $\buff \leftarrow (s, a, s', r)$
            \State Update $Q_\theta$ and $\policy_\theta$, sampling from $\buff$
  	\Until{converged}
  	}
  	\end{algorithmic}
\end{algorithm}
